MyDigiTwin: A Privacy-Preserving Framework for Personalized Cardiovascular Risk Prediction and Scenario Exploration

Cardiovascular disease (CVD) remains a leading cause of death, and primary prevention through personalized interventions is crucial. This paper introduces MyDigiTwin, a framework that integrates health digital twins with personal health environments to empower patients in exploring personalized health scenarios while ensuring data privacy. MyDigiTwin uses federated learning to train predictive models across distributed datasets without transferring raw data, and a novel data harmonization framework addresses semantic and format inconsistencies in health data. A proof-of-concept demonstrates the feasibility of harmonizing and using cohort data to train privacy-preserving CVD prediction models. This framework offers a scalable solution for proactive, personalized cardiovascular care and sets the stage for future applications in real-world healthcare settings.

==> abstract.tex <==
Cardiovascular disease (CVD) continues to be a significant public health issue, with early detection and prevention being crucial in alleviating healthcare pressures. This paper introduces MyDigiTwin, a framework that integrates Digital Twin technology with Personal Health Environments to facilitate personalized cardiovascular risk prediction and proactive health management. By utilizing population-based predictive models within a federated learning architecture, MyDigiTwin guarantees privacy-preserving data handling, obviating the necessity for sharing raw patient data across institutions. The framework addresses crucial challenges in digital health, such as data fragmentation, limited patient engagement, and regulatory constraints. It accomplishes this by harmonizing data utilizing FHIR-based standards, thereby enabling consistent and scalable model development. An end-to-end proof of concept demonstrates the feasibility of employing federated data for predictive modeling, enhancing the discriminative performance of cardiovascular risk models across multiple datasets. MyDigiTwin enables patients to simulate health scenarios, thereby promoting lifestyle changes to mitigate risks. The framework lays the groundwork for the broader adoption of personalized healthcare technologies, with an emphasis on transparency, security, and interoperability. Although challenges persist in scaling to heterogeneous datasets and improving accessibility, MyDigiTwin represents a critical advancement towards revolutionizing cardiovascular care through patient-centered, data-driven innovations. Future research will investigate model validation in real-world settings and address the challenges posed by statistical and demographic diversity in data integration.
